Privacy-Utility Tradeoff Based on $\alpha$-lift

Information density and its exponential form, known as lift, play a central role in information privacy leakage measures. $\alpha$-lift is the power-mean of lift, which is tunable between the worst-case measure max-lift ($\alpha=\infty$) and more relaxed versions ($\alpha<\infty$). This paper investigates the optimization problem of the privacy-utility tradeoff (PUT) where $\alpha$-lift and mutual information are privacy and utility measures, respectively. Due to the nonlinear nature of $\alpha$-lift for $\alpha<\infty$, finding the optimal solution is challenging. Therefore, we propose a heuristic algorithm to estimate the optimal utility for each value of $\alpha$, inspired by the optimal solution for $\alpha=\infty$ and the convexity of $\alpha$-lift with respect to the lift, which we prove. The numerical results show the efficacy of the algorithm and indicate the effective range of $\alpha$ and privacy budget $\varepsilon$ with good PUT performance.

==> cover.tex <==
Dear Editor-in-Chief,

Please find attached our manuscript entitled ``Privacy-Utility Tradeoff Based on alpha-lift" for possible publication in the IEEE Signal Processing Letters. 

We confirm that this paper has not been submitted to any other conference or journal previously or currently. However, we have posted a preprint of this work onto ArXiv on 11 June 2024. Compared to the ArXiv version, we have streamlined the algorithm and improved the numerical results.

Please feel free to contact us if you require more information. Thank you for your consideration and for handling this submission.

Kind regards,

Mohammad Amin Zarrabian and Parastoo Sadeghi
